STAG4D: Spatial-Temporal Anchored Generative 4D Gaussians

Recent progress in pre-trained diffusion models and 3D generation have spurred interest in 4D content creation. However, achieving high-fidelity 4D generation with spatial-temporal consistency remains a challenge. In this work, we propose STAG4D, a novel framework that combines pre-trained diffusion models with dynamic 3D Gaussian splatting for high-fidelity 4D generation. Drawing inspiration from 3D generation techniques, we utilize a multi-view diffusion model to initialize multi-view images anchoring on the input video frames, where the video can be either real-world captured or generated by a video diffusion model. To ensure the temporal consistency of the multi-view sequence initialization, we introduce a simple yet effective fusion strategy to leverage the first frame as a temporal anchor in the self-attention computation. With the almost consistent multi-view sequences, we then apply the score distillation sampling to optimize the 4D Gaussian point cloud. The 4D Gaussian spatting is specially crafted for the generation task, where an adaptive densification strategy is proposed to mitigate the unstable Gaussian gradient for robust optimization. Notably, the proposed pipeline does not require any pre-training or fine-tuning of diffusion networks, offering a more accessible and practical solution for the 4D generation task. Extensive experiments demonstrate that our method outperforms prior 4D generation works in rendering quality, spatial-temporal consistency, and generation robustness, setting a new state-of-the-art for 4D generation from diverse inputs, including text, image, and video.

==> backups/backup_adaptive_densify.tex <==
\textbf{Adaptive Densification}
[figures here]
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{sec/figs/fig_adaptive_threshold.jpg}
  \vspace{-0.2in}
  \caption{\textbf{Ablation Study on Adaptive Densification.} 
  }
  \vspace{-0.2in}
  \label{fig:photo_cust_compare}
\end{figure}

==> backups/backup_multiview_sds.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{sec/figs/fig_mv_sds2.jpg}
  \vspace{-0.2in}
  \caption{\textbf{Ablation Study on Multiview SDS.} 
  }
  \vspace{-0.2in}
  \label{fig:photo_cust_compare}
\end{figure}

==> backups/backup_qualitative_comparison.tex <==
\begin{figure*}[ht]
  \includegraphics[width=1.0\linewidth]{sec/figs/fig_comparison.jpg}
  \vspace{-0.2in}
  \caption{
  \textbf{Qualitative comparison
  }}
  \label{fig:qualitative}
  \vspace{-0.2in}
\end{figure*}

==> backups/backup_timemix.tex <==
\yanqin{[description here]}
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{sec/figs/fig_temportal_consist_on recon2.jpg}
  \vspace{-0.2in}
  \caption{\textbf{Ablation Study on TimeMix for Reconstruction} 
  }
  \vspace{-0.2in}
  \label{fig:photo_cust_compare}
\end{figure}

==> backups/backup_user_study.tex <==
\begin{table}[]
\centering
\caption{\textbf{User Study \& Metrics}}
\vspace{-0.1in}
\begin{tabular}{@{}lccccc@{}}
\toprule
            & Vis. & Cons. & FID  & Train & Ren. \\
\cite{jiang2023consistent4d} & 76.1  & 80.4     & ?  & 150  &  ? \\
Ours        & 89.2  & 92.2  & 136(?) & 30  & 150  \\ \bottomrule
\end{tabular}
\vspace{-0.15in}
\label{tab:quantitative}
\end{table}

==> backups/backup_zero123_plus_plus_failure_examples.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{sec/figs/fig_temporal_consist_example2.jpg}
  \vspace{-0.2in}
  \caption{\textbf{Zero123++ Failure Examples.} 
  }
  \vspace{-0.2in}
  \label{fig:zero123_example}
\end{figure}

==> sec/abstract.tex <==
\begin{abstract}

Recent advancements in large-scale pre-trained image diffusion models and image-to-3D generation methods have spurred interest in 4D scene generation from monocular video input. However, achieving high-fidelity and temporally consistent 4D generation remains a challenge for current video-to-4D methods. This paper presents a novel framework that combines a pre-trained image diffusion model with dynamic 3D Gaussian splatting for high-fidelity video-to-4D generation. 
The 4D Gaussian spatting is specially tailored for the video-to-4D task, where an adaptive densification strategy is proposed to mitigate the unstable Gaussian gradient, significantly improving the generation quality and robustness. 
To address the spatial consistency of the final generation, we employ a multi-view diffusion model that takes the corresponding input frame as an anchor for cross-view attention computation. 
Crucially, for temporal consistency, we introduce TimeMix, a fusion technique incorporating the first frame information of the video into the multi-view diffusion process, which significantly boosts the consistency temporally and the overall generation quality.
% Experimental results on public datasets demonstrate substantial improvements in rendering quality and temporal consistency, including a $5\times$ faster training and rendering speed, while consistently achieving comparable or superior results to prior leading methods.
Extensive experiments on public datasets demonstrate substantial improvements brought by each component of the proposed method. Our method outperforms prior works in 4D rendering quality, spatial-temporal consistency, and generation robustness, setting a new state-of-the-art for the task of video-to-4D generation. 

\end{abstract}

==> sec/preliminary.tex <==
\section{Preliminary}



\subsection{Image Diffusion Models in 3D Generation}
% general intro
Optimization-based 3D generation models usually require knowledge distillation from 2D image diffusion models.
% image diffusion models
In early works, standard text-to-image models, such as stable diffusion and deepfloyd-if, are adopted due to easy access. However, since these models lacks 3D awareness, the generated results often suffer from multi-janus problem.
%
To overcome the multi-janus problem, researchers embed the camera pose information to image diffusion models and finetune them with multi-view images rendered from large-scale 3D datasets.
%
Zero123~\cite{liu2023zero} and Zero123++~\cite{shi2023zero123++} are two representative of such image diffusion models.
%

% zero123
Given the input view image $\mathbf{I}_{in}$ and the relative camera pose $(\mathbf{R}, \mathbf{T})$ between the input and the target view, zero123 is capable of predicting the target view image. This image-to-image diffusion model, denoted by $\phi$, is utilized to calculate SDS loss for 3D generation as follows:
\begin{equation}
    \nabla_{\theta} \mathcal{L}_{SDS}(\phi, \mathbf{x}) = \mathbb{E}_{t, \epsilon} \left [ \omega(t)(\hat{\epsilon}_\theta(\mathbf{z}_t;\mathbf{I}_{in}, \mathbf{R}, \mathbf{T}, t) - \epsilon) \frac{\partial \mathbf{x}}{\partial \theta}\right ],
\end{equation}
where $\theta$ represents parameters of 3D representation, e.g., NeRF, $\mathbf{x}$ and $\mathbf{z}$ are rendering and noisy rendering images, and $t$ is the timestamp in diffusion. $\epsilon$ denotes noise and $\omega$ is a weighted function.
% zero123++
Zero123 only generates the image of one target view at a time so multi-view images generated by it suffer from spatial inconsistency. To overcome this inconsistency, the authors propose Zero123++, which allows ineteraction between multi-view predictions and are able to output images from six different target views at once. However, since the relative positions between input view and output views are fixed, and the output views are quite sparse, neither this model nor its outputs could be directly applied to 3D tasks.
% relate to ours
In this work, we find a way to take advantage of multi-view consistent images generated by Zero123++ and the key idea is inserting multi-view images into SDS loss of Zero123, which will be explained in Sec.~\ref{sec: method}.

\subsection{3D Gaussian Splatting for Reconstruction}
% general intro




==> sec/teaser.tex <==
\begin{teaserfigure}
    \includegraphics[width=\textwidth]{img/teaser.png}
    \label{fig:teaser}
\end{teaserfigure}

==> tab/ablation_attention.tex <==

  % Second minipage for the second table
  %\begin{minipage}[t]{0.35\textwidth}
  %  \centering
  %  \begin{adjustbox}{width=\textwidth}
  %  \begin{tabular}{@{}lcccc@{}}
  %    \toprule
  %    & \multicolumn{4}{c}{Evaluation Metrics} \\
  %     & CLIP $\uparrow$ & LPIPS $\downarrow$ & FID-VID $\downarrow$ & FVD $\downarrow$ \\
  %    \midrule
  %    No & & & & \\
  %    Cross Frame Attention & & & & \\
  %    ours & & & &  \\
  %    \bottomrule
  %  \end{tabular}
  %  \end{adjustbox}
  %  \vspace{0.075cm}
  %  \caption{Comparison of different temporal attentions.}
  %  \label{tab:temporal_attn}
  %\end{minipage}


==> tab/user_study.tex <==
\begin{table}[]
\centering
\vspace{-0.1in}
\begin{tabular}{@{}lccc@{}}
\toprule
            & Vis. & Cons. & FID   \\
\hline
Consistent4D & 28.6\% & 28.6\% & 35.7\%    \\
4DGen & 0\% & 0\% & 0\%  \\
Ours        & 71.4\% & 71.4\% & 64.3\% \\ 
\bottomrule
\end{tabular}
\caption{User study on the best-performing 4D-to-Video generation methods. We ask respondents to compare the three methods on visual quality, temporal consistency, and generation consistency to input video. Totally 31 respondents were invited and the proposed method demonstrated clear popularity compared to the alternatives.}
\label{tab:user_study}
\end{table}
